From Tokens to Concepts: Leveraging SAE for SPLADE

Learned Sparse IR models, such as SPLADE, offer an excellent efficiency-effectiveness tradeoff. However, they rely on the underlying backbone vocabulary, which might hinder performance (polysemicity and synonymy) and pose a challenge for multi-lingual and multi-modal usages. To solve this limitation, we propose to replace the backbone vocabulary with a latent space of semantic concepts learned using Sparse Auto-Encoders (SAE). Throughout this paper, we study the compatibility of these 2 concepts, explore training approaches, and analyze the differences between our SAE-SPLADE model and traditional SPLADE models. Our experiments demonstrate that SAE-SPLADE achieves retrieval performance comparable to SPLADE on both in-domain and out-of-domain tasks while offering improved efficiency.

==> tab/main_result/main_res_beir.tex <==
% This is the table with the full info.
\begin{table*}[!ht]
    \centering
    \renewcommand\cellalign{l}
    \caption{The evaluation results for SAE-SPLADE ($k=8$, TopK SAE) and baseline models on 13 BEIR dataset. The best metrics are in \textbf{bold}. 
    }
    \resizebox{\linewidth}{!}{
    \begin{tabular}{m{2.3cm}|C{0.6cm}C{0.6cm}C{0.6cm}C{0.6cm}C{0.6cm}C{0.6cm}C{0.6cm}C{0.6cm}C{0.6cm}C{0.6cm}C{0.6cm}C{0.6cm}C{0.6cm}|C{0.6cm}}
        \Xhline{1pt}
        \textbf{model} & \textbf{\small{AR.}} & \textbf{\small{CF.}} & \textbf{\small{DB.}} & \textbf{\small{FV.}} &  \textbf{\small{FQ.}} & \textbf{\small{HQ.}} & \textbf{\small{NF.}} & \textbf{\small{NQ.}} & \textbf{\small{QU.}} & \textbf{\small{SD.}} & \textbf{\small{SF.}} & \textbf{\small{TC.}} & \textbf{\small{TO.}} & \textbf{\small{Avg.}}\\
        \Xhline{1pt}
        \multicolumn{15}{l}{\textit{Multi Vector Dense Model}} \\ \hline
        % ANCE & 41.5 & 19.8 & 28.1 & 66.9 & 29.5 & 45.6 & 23.7 & 44.6 & 85.2 & 12.2 & 50.7 & 65.4 & 24.0 & 41.3 \\
        ColBERTv2\scriptsize{base} & 46.3 & 17.6 & 44.6 & 78.5 & 35.6 & 66.7 & 33.8 & 56.2 & 85.2 & 15.4 & 69.3 & 73.8 & 26.3 & 50.0 \\
        \Xhline{1pt}
        \multicolumn{15}{l}{\textit{Sparse Model}} \\ \hline
        BM25 & 39.7 & 16.5 & 31.8 & 65.1 & 23.6 & 63.3 & 32.2 & 30.5 & 78.9 & 14.9 & 67.9 & 59.5 & 44.2 & 43.7 \\
        SPLADEv3 & 48.4 & 22.8 & 42.6 & 79.6 & 33.9 & 67.8 & 34.8 & 54.9 & 81.7 & 14.8 & 68.5 & 70.0 & 30.1 & 50.0 \\
        \Xhline{1pt}
        \multicolumn{15}{l}{\textit{Ours}} \\ \hline
        SPLADE & 46.3 & 20.3 & 43.8 & 77.7 & 31.4 & 68.6 & 33.4 & 52.8 & 83.3 & 14.5 & 65.6 & 65.9 & 31.4 & 48.8 \\
        SAE-SPLADE \scriptsize{k=4} & 46.3 & 19.7 & 42.2 & 76.1 & 31.6 & 66.7 & 33.3 & 50.8 & 82.9 & 14.4 & 63.7 & 70.1 & 32.9 & 48.5 \\
        SAE-SPLADE \scriptsize{k=8} & 47.0 & 20.8 & 43.3 & 77.7 & 32.7 & 67.6 & 33.3 & 52.1 & 84.0 & 14.2 & 64.4 & 68.6 & 33.3 & 49.2 \\
        SAE-SPLADE \scriptsize{k=16} & 47.4 & 21.3 & 43.9 & 77.8 & 32.9 & 68.1 & 33.6 & 53.2 & 84.8 & 14.5 & 65.1 & 68.8 & 33.8 & 49.6 \\
        \Xhline{1pt}
    \end{tabular}
    }
    \label{tab:sae_splade_main_in_domain}
\end{table*}



==> tab/main_result/main_res_in_domain.tex <==
% full in-domain.
\begin{table}[!ht]
    \centering
    \renewcommand\cellalign{l}
    \caption{The evaluation results for SAE-SPLADE ($k=8$, TopK SAE) and baseline models on in-domain MS MARCO dataset. We report the metric reflecting the effectiveness (MRR@10 for dev-small, nDCG@10 for TREC-DL mean, including TREC DL19 and TREC DL20), and efficiency (QD-flops, Avg. D Len), and the metric $s_{\operatorname{eval}}$ that reflecting both. The best metrics are in \textbf{bold}. 
    }
    \resizebox{\linewidth}{!}{
    \begin{tabular}{m{2.4cm}|C{1.1cm}C{1cm}C{1cm}|C{1.3cm}C{1.35cm}|C{0.8cm}}
        \Xhline{1pt}
        \textbf{model} & \textbf{\small{Dev set}} & \textbf{\small{DL19}} & \textbf{\small{DL20}} &  \textbf{\small{QD-flops}} & \textbf{\small{Avg. D Len}} & \small{$\Delta\EEscore$} \\
        \Xhline{1pt}
        \multicolumn{7}{l}{\textit{(Single or Multi Vector) Dense Model}} \\ \hline
        % ANCE & 33.0 & 64.5 & 64.5 & - & - & - \\
        SimLM & \textbf{41.1} & 71.4 & 69.7 & - & - & - \\
        ColBERTv2\scriptsize{distilbert} & 38.3 & 73.5 & 73.6 & - & - & - \\
        ColBERTv2\scriptsize{base} & 39.7 & 74.5 & \textbf{75.6} & - & - & - \\
        \Xhline{1pt}
        \multicolumn{7}{l}{\textit{Sparse Model}} \\ \hline
        BM25 & 18.3 & 50.6 & 48.0 & \textbf{0.13} & \textbf{39} & - \\
        CL-SR & 36.8 & 68.6 & 63.4 & 0.74 & 65 & - \\
        % SPLADEv2 & 35.8 & 70.6 & 68.7 & 1.39 & - & - \\
        SPLADEv3 & 38.7 & \textbf{75.2} & 74.4 & 1.40 & 165 & - \\
        \Xhline{1pt}
        \multicolumn{7}{l}{\textit{Ours}} \\ \hline
        SPLADE & 37.7 & 73.0 & 71.0 & 1.47 & 118 & - \\
        SAE-SPLADE \scriptsize{$k=4$} & 37.1 & 71.1 & 71.8 & 0.33 & 66 & - \\
        SAE-SPLADE \scriptsize{$k=8$} & 37.6 & 72.2 & 72.0 & 0.67 & 109 & - \\
        SAE-SPLADE \scriptsize{$k=16$} & 38.2 & 73.2 & 71.3 & 1.37 & 191 & - \\
        \Xhline{1pt}
    \end{tabular}
    }
    \label{tab:sae_splade_main_in_domain}
\end{table}

==> tab/main_result/main_res_lotte.tex <==
% This is the table with the full info.
\begin{table}[!ht]
    \centering
    \renewcommand\cellalign{l}
    \caption{The evaluation results for SAE-SPLADE ($k=8$, TopK SAE) and baseline models on LoTTE search test set. The best metrics are in \textbf{bold}. 
    }
    \resizebox{\linewidth}{!}{
    \begin{tabular}{m{2.3cm}|C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}C{0.7cm}|C{0.7cm}}
        \Xhline{1pt}
        \textbf{model} & \textbf{\small{Wrt.}} & \textbf{\small{Rcr.}} & \textbf{\small{Sci.}} &  \textbf{\small{Tch.}} & \textbf{\small{LS.}} & \textbf{\small{Avg.}} \\
        \Xhline{1pt}
        \multicolumn{7}{l}{\textit{(Single or Multi Vector) Dense Model}} \\ \hline
        ANCE & 74.4 & 64.7 & 53.6 & 59.6 & 82.3 & 67.0 \\
        ColBERTv2\scriptsize{distilbert} & 78.3 & 71.7 & 55.4 & 64.9 & 82.8 & 70.6 \\
        ColBERTv2\scriptsize{base} & 80.1 & 72.3 & 56.7 & 66.1 & 84.7 & 72.0 \\
        \Xhline{1pt}
        \multicolumn{7}{l}{\textit{Sparse Model}} \\ \hline
        BM25 & 60.3 & 56.5 & 32.7 & 41.8 & 63.8 & 51.0 \\
        % SPLADEv2 & 72.1 & 67.8 & 53.2 & 60.1 & 80.0 \\
        SPLADEv3 & - & - & - & - & - & 70.3 \\
        \Xhline{1pt}
        \multicolumn{7}{l}{\textit{Ours}} \\ \hline
        SPLADE & 76.1 & 69.2 & 55.2 & 61.2 & 82.3 & 68.9 \\
        SAE-SPLADE \scriptsize{k=4} & 75.4 & 68.5 & 54.9 & 62.1 & 80.3 & 68.2\\
        SAE-SPLADE \scriptsize{k=8} & 76.7 & 68.0 & 53.3 & 63.6 & 82.3 & 68.8 \\
        SAE-SPLADE \scriptsize{k=16} & 77.8 & 69.7 & 55.1 & 62.4 & 81.6 & 69.4 \\
        \Xhline{1pt}
    \end{tabular}
    }
    \label{tab:sae_splade_main_in_domain}
\end{table}


==> tab/train_qry_norm_ab.tex <==
\begin{table}[!ht]
    \centering
    \caption{The evaluation results for SAE-SPLADE ($k=8$, TopK SAE) with or without the
    normalization of SAE and pretrain with or without the query text.}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{m{1cm}m{1cm}|C{1cm}C{1cm}C{1cm}|C{1cm}C{1cm}|C{1cm}}   
        \Xhline{1pt}  
        \footnotesize{Norm. SAE} & \footnotesize{Train Qry.} &  \small{dev-small} & \small{TREC-DL}
        & \small{OoD mean} & \small{QD-flops} &  \small{Avg. D Len} & \small{$\Delta\EEscore$}\\ 
        \Xhline{1pt}  
        \rowcolor{lightgray} \xmark & \xmark & \textbf{37.6} & 72.1 & 68.8 & 0.67 & 109 &
        \textbf{0.889} \\
        \Xhline{1pt}  
        \color{gray}{\xmark} & \cmark & 37.2 & \textbf{72.4} & \textbf{69.0} & \textbf{0.66} & 111 &
        0.870 \\
        \cmark & \color{gray}{\xmark} & 37.6 & 71.3 & 68.7 & 0.67 & \textbf{108} & 0.889 \\
        \cmark & \cmark & 37.6 & 71.3 & 68.9 & 0.68 & 112 & 0.888 \\
        \Xhline{1pt}
    \end{tabular}
    } 
    \label{tab:sae_splade_qry_norm_ab}
\end{table}

==> tab/variants_k/htopk_k_ab.tex <==
\begin{table}[!ht]
    \centering
    \caption{The ablation results of Hierarchical TopK SAE-SPLADE where the SAE is trained with
    $k=32$ while SPLADE is trained with various $k$. Meanwhile, we also tested
    the three best performing $k$ values in term of effectiveness and efficiency (e.g, $k=4, 8, 16$) with a higher SAE pretraining $k$. }
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{C{1cm}C{1cm}|C{1cm}C{1cm}C{1cm}|C{1cm}C{1cm}|C{1cm}}
        \Xhline{1pt}
        $k_{\operatorname{SAE}}$ & $k_{\operatorname{SPLADE}}$ & \small{dev-small} & \small{TREC-DL}
        & \small{OoD mean} & \small{QD-flops} &  \small{Avg. D Len} & \small{$\Delta\EEscore$} \\ 
        \Xhline{1pt}
        \multirow{6}{*}{32} & 2 & 34.0 & 67.0 & 65.4 & \textbf{0.13} & \textbf{31} & 0.730 \\ 
        & 4 & 37.0 & 71.2 & 68.1 & 0.30 & 62 & 0.867 \\
        & 8 & 37.5 & 71.2 & 69.2 & 0.64 & 117 & 0.883\\
        & 16 & 37.8 & 71.6 & 69.5 & 1.43 & 208 & \textbf{0.884}\\
        & 32 & 37.9 & 71.7 & 70.0 & 2.71 & 308 & 0.838 \\
        & Full & \textbf{38.0} & \textbf{71.9} & \textbf{70.3} & 4.57 & 387 & 0.672\\
        \Xhline{1pt}
        \multirow{3}{*}{128} & 4 & 37.0 & 71.2 & 67.5 & 0.32 & 56 & 0.867 \\ 
        & 8 & 37.3 & 71.8 & 69.0 & 0.72 & 106 & 0.874 \\
        & 16 & 38.0 & 71.9 & 69.6 & 1.52 & 192 & 0.890 \\
        \Xhline{1pt}
    \end{tabular}
    }
    \label{tab:sae_splade_htopk_ab}
\end{table}

==> tab/variants_k/mtopk_k_ab.tex <==
\begin{table}[!ht]
    \centering
    \caption{The ablation results of Matryoshka TopK SAE-SPLADE where the SAE is trained with
    $k=32$ while SPLADE is trained with various $k$. We pretrain the Matryoshka SAE with
    $k=32$ and finetune different SPLADE model with different $k$ values.}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{C{1cm}C{1cm}|C{1cm}C{1cm}C{1cm}|C{1cm}C{1cm}|C{1cm}}
        \Xhline{1pt}
        $k_{SAE}$ & $k_{SPLADE}$ & \small{dev-small} & \small{TREC-DL mean} & \small{OoD mean} &
        \small{QD-flops} &  \small{Avg. D Len} & \small{$\Delta\EEscore$}\\ 
        \Xhline{1pt}
        \multirow{6}{*}{32} & 2 & 34.5 & 67.5 & 65.2 & \textbf{0.14} & \textbf{32} & 0.753 \\
        & 4 & 37.0 & 71.5 & 67.8 & 0.32 & 66 & 0.864\\
        & 8 & 37.5 & 72.0 & 68.9 & 0.73 & 124 & \textbf{0.881}\\
        & 16 & 37.7 & 72.2 & 69.6 & 1.50 & 209 & 0.874\\
        & 32 & 37.7 & 72.8 & 69.6 & 2.60 & 298 & 0.834\\
        & Full & \textbf{37.7} & \textbf{73.1} & \textbf{70.0} & 4.84 & 408 & 0.620\\
        \Xhline{1pt}
    \end{tabular}
    } 
    \label{tab:sae_splade_mtopk_ab}
\end{table}

==> tab/variants_k/topk_k_ab.tex <==
\begin{table}[!ht]
    \centering
    \caption{The ablation results of TopK SAE-SPLADE for various $k$. 
    All SAE-SPLADE models are pretrained using a TopK SAE with the same $k$ value, except for the full-width setting, where pretraining is performed with a TopK SAE using $k=8$.
    % \todo{Maybe we can add the values of the DistilColBERT and bm25 up and down, which shows that if we push our model extremely efficient, it could have better performance than bm25. Meanwhile our most effective model could also achieve the performance of ColBERTv2. }
    }
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{C{1cm}|C{1cm}C{1cm}C{1cm}|C{1cm}C{1cm}|C{1cm}}    
        \Xhline{1pt}   
        $k_{SPLADE}$ & \small{dev-small} & \small{TREC-DL} & \small{OoD mean} & \small{QD-flops} &
        \small{Avg. D Len} & \small{$\Delta\EEscore$}\\ 
        \Xhline{1pt}
        2 & 35.2 & 67.6 & 66.0 & \textbf{0.15} & \textbf{37} & 0.785 \\
        4 & 37.1 & 71.5 & 68.2 & 0.33 & 66 & 0.868 \\
        8 & 37.6 & 72.1 & 68.8 & 0.67 & 109 & 0.889 \\
        16 & \textbf{38.2} & 72.3 & 69.4 & 1.37 & 191 & \textbf{0.904} \\ 
        32 & 37.8 & 72.6 & \textbf{70.6} & 2.67 & 316 & 0.837 \\
        Full & 38.1 & \textbf{73.5} & 70.3 & 5.36 & 369 & 0.549 \\ 
        \Xhline{1pt}
    \end{tabular}
    }
    \label{tab:sae_splade_topk_ab}
\end{table}

==> tab/vocab_size.tex <==
\begin{table}[!ht]
    \centering
    \caption{The ablation results of the size of the Vocabulary.}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{m{0.5cm}|C{1.2cm}C{1.2cm}C{1.3cm}|C{1.2cm}C{1.4cm}|C{1cm}}
        \Xhline{1pt}
        $M$ & \small{dev-small} & \small{TREC-DL} & \small{OoD mean} & \small{QD-flops} &
        \small{Avg. D Len} & \small{$\Delta\EEscore$}\\
        \Xhline{1pt}
        $2^{15}$ & 37.8 & 71.9 & 68.8 & 0.66 & 107 & \textbf{0.898} \\
        \rowcolor{lightgray} $2^{16}$ & 37.6 & 72.1 & 68.8 & 0.66 & 111 & 0.889 \\
        $2^{17}$ & 37.6 & 72.3 & 68.6 & 0.66 & 113 & 0.889 \\
        \Xhline{1pt}
    \end{tabular}
    }
    \label{tab:sae_splade_vocab_size}
\end{table}
